Algorithmic Learning Foundations for Common Law

This paper looks at a common law legal system as a learning algorithm, models specific features of legal proceedings, and asks whether this system learns efficiently. A particular feature of our model is explicitly viewing various aspects of court proceedings as learning algorithms. This viewpoint enables directly pointing out that when the costs of going to court are not commensurate with the benefits of going to court, there is a failure of learning and inaccurate outcomes will persist in cases that settle. Specifically, cases are brought to court at an insufficient rate. On the other hand, when individuals can be compelled or incentivized to bring their cases to court, the system can learn and inaccuracy vanishes over time.

==> algorithm/alg-without-incentives.tex <==
\begin{algorithm}
\caption{Original Algorithm in \cite{lattimore2020bandit} for PMP}
\begin{algorithmic}
\STATE{\textbf{Input:}} $\varepsilon,\eta$
\FOR{$t = 1,2,\dots, n$}
\STATE Compute exponential weight distribution $Q_t$ by 
$$
Q_t(a) = \frac{\exp(-\eta\sum_{s=1}^{t-1} y_s(a))}{\sum_{b \in [k]} \exp(-\eta\sum_{s=1}^{t-1} y_s(b))}
$$
\STATE Solve for the exploration distribution $P_t$ and estimation function $f_t$ with $Q_t$ and $\epsilon$ %and accumulated extra exploration rate $e_t$.
\STATE Sample $A_t \sim P_t$ and observe $\sigma_t$
\STATE Update $y_t = f_t(A_t,\sigma_t)/P_{t}(A_t)$.
%\STATE Update $e_t$ according to $P_t$ and incentives of agents.  
%\STATE Update the learning rate $\eta_t$ 
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> algorithm/algo-with-incentives.tex <==
\begin{algorithm}
\caption{Algorithm with Incentives}
\begin{algorithmic}
\STATE{\textbf{Input:}} $\varepsilon,\eta_1$
\FOR{$t = 1,2,\dots, n$}
\STATE Compute exponential weight distribution $Q_t$ by 
$$
Q_t(a) = \frac{\exp(-\eta_t\sum_{s=1}^{t-1} y_s(a))}{\sum_{b \in [k]} \exp(-\eta_t\sum_{s=1}^{t-1} y_s(b))}
$$
\STATE Solve the exploration distribution $P_t$ and estimation function $f_t$ with $Q_t,\epsilon$ and accumulated extra exploration rate $e_t$.
\STATE Sample $A_t \sim P_t$ and observe $\sigma_t$
\STATE Update $y_t = f_t(A_t,\sigma_t)/P_{t}(A_t)$.
\STATE Update $e_t$ according to $P_t$ and incentives of agents.  
\STATE Update the learning rate $\eta_t$ 
\ENDFOR
\end{algorithmic}
\end{algorithm}
